Accelerating Grasp Exploration by Leveraging Learned Priors

The ability of robots to grasp novel objects has industry applications in e-commerce order fulfillment and home service. Data-driven grasping policies have achieved success in learning general strategies for grasping arbitrary objects. However, these approaches can fail to grasp objects which have complex geometry or are significantly outside of the training distribution. We present a Thompson sampling algorithm that learns to grasp a given object with unknown geometry using online experience. The algorithm leverages learned priors from the Dexterity Network robot grasp planner to guide grasp exploration and provide probabilistic estimates of grasp success for each stable pose of the novel object. We find that seeding the policy with the Dex-Net prior allows it to more efficiently find robust grasps on these objects. Experiments suggest that the best learned policy attains an average total reward 64.5% higher than a greedy baseline and achieves within 5.7% of an oracle baseline when evaluated over 300,000 training runs across a set of 3000 object poses.

==> includes/0-macros.tex <==
\usetikzlibrary{backgrounds}
\numberwithin{equation}{section} 
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\ceq}{\ensuremath{\mathrel{\stackrel{\mathrm{def}}{=}}}} 
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\rd}{{\mathrm d}}
\newcommand{\p}{\partial}
\tikzstyle{every node}=[font=\small]
%%\usepackage{filemod}
\newcommand{\includetikz}[2]{%
\tikzsetnextfilename{#2}%
    \filemodCmp{#1#2.tikz}{#1tikz/#2.pdf}%
        {\tikzset{external/remake next}}{}%
    \input{#1#2.tikz}%
}

\captionsetup{font={footnotesize}}

%\usepackage{tabularx}
%\usepackage{pbox}
%\usepackage{ragged2e}
%\usepackage{multirow}
%\usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]

\newcolumntype{L}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{R}[1]{>{\RaggedLeft\hspace{0pt}}p{#1}}

\DeclareMathOperator{\J}{J} 
\DeclareMathOperator{\clamp}{clamp} 
\DeclareMathOperator{\interior}{int} 
\DeclareMathOperator{\D}{D} 
\DeclareMathOperator{\Div}{div} 
\DeclareMathOperator{\Sgn}{Sgn} 
\DeclareMathOperator{\Hom}{Hom} 
\DeclareMathOperator{\rank}{rank} 
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\Area}{Area}
\DeclareMathOperator{\dVol}{dVol}
\DeclareMathOperator{\supp}{supp} 
\DeclareMathOperator{\Int}{Int} 
\DeclareMathOperator{\Conv}{Conv} 
\DeclareMathOperator{\Cone}{Cone} 
\DeclareMathOperator{\Ker}{Ker} 
\DeclareMathOperator{\Span}{Span} 
\DeclareMathOperator{\Min}{Min} 
\newcommand{\bone}{\mathbf{1}}
\DeclareMathOperator{\tr}{tr} 
\newcommand{\bR}{\mathbb{R}} 
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}} 
\newcommand{\bB}{\mathbb{B}} 
\newcommand{\bbT}{\mathbb{T}} 
\newcommand{\bN}{\mathbb{N}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cO}{\mathcal{O}} 
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cKG}{\mathcal{KG}}
\renewcommand{\phi}{\varphi}
\renewcommand{\div}{\mbox{div}}
\newcommand{\ve}{\varepsilon}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\diff}[4]{\left.\left.\frac{\operatorname{d}}{\operatorname{d}#1}\right.^{#2}#3\right|_{#4}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

\newcommand{\furlp}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/papers/#1.pdf}{D}}}
\newcommand{\furlb}[1]{\colorbox{blue!10}{\href{run:/home/fulong/academia/library/books/#1.pdf}{D}}}
\newcommand{\fcitep}[1]{\cite{#1}\mbox{\furlp{#1}}}
\newcommand{\fciteb}[1]{\cite{#1}\mbox{\furlb{#1}}}
% we can now use cite as before
% misc defines
\newcommand{\energy}{U}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\hbx}{\hat{\mathbf{x}}}
\newcommand{\bbx}{\bar{\mathbf{x}}}
\newcommand{\sbx}{\mathbf{x}^{\star}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\hbb}{\hat{\mathbf{b}}}
\newcommand{\hbn}{\hat{\mathbf{n}}}
\newcommand{\bbb}{\bar{\mathbf{b}}}
\newcommand{\hbu}{\hat{\mathbf{u}}}
\newcommand{\bbu}{\bar{\mathbf{u}}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mZ}{\mathcal{Z}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mQ}{\mathcal{Q}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\hmX}{\hat{\mathcal{X}}}
\newcommand{\hmU}{\hat{\mathcal{U}}}
\newcommand{\bmX}{\bar{\mathcal{X}}}
\newcommand{\bmU}{\bar{\mathcal{U}}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\hbpsi}{\hat{\boldsymbol \psi}}
\newcommand{\bPsi}{\boldsymbol \Psi}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\sS}[1]{\sqrt{\Sigma_{#1}}}
\newcommand{\shS}[1]{\sqrt{\hat{\Sigma}_{#1}}}
\newcommand{\sd}{\texttt{sd}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Tr}{tr}
\DeclareMathOperator{\st}{s.t.}
\DeclareMathOperator{\dt}{dt}
\DeclareMathOperator{\Vect}{vec}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\argmin}{arg\,min}

\newcommand{\specialcell}[2][c]{ \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\limit}[1] {\underset{#1}{\text{lim }}}
\newcommand{\infimum}[1] {\underset{#1}{\text{inf }}}
\newcommand{\supremum}[1] {\underset{#1}{\text{sup }}}
\newcommand{\maximum}[1] {\underset{#1}{\text{max }}}
\newcommand{\minimum}[1] {\underset{#1}{\text{min }}}
\newcommand{\myargmax}[1] {\underset{#1}{\text{argmax }}}
\newcommand{\myargmin}[1] {\underset{#1}{\text{argmin }}}
\newcommand{\expect}[1] {\mathbb{E}\left[#1\right]}

==> includes/4.5-analysis.tex <==
\section{Grasp Exploration Analysis}
\todo{Ashwin: seems like we may not want to frame this as a contextual bandits problem but instead as a set of independent bandit problems with some (possibly) non-stationary distribution which determines how many rounds of learning you get for each problem}

We first provide results on the probability of missing a particular stable pose under any stationary policy. We then provide a bound on the expected total regret for the learned Thompson sampling policy if the object is dropped after every timestep. All proofs are included in the supplementary material.

\subsection{Pose Coverage Analysis}
\label{subsec:pose-coverage-analysis}

\todo{Ashwin: Maybe should add a separate definition for $\eta^\pi_i$ and its analogue for prob of grasp success on stable pose $P^i$, $\gamma^\pi_i$ since this will be needed for analysis of the expected num occurrences of each stable pose + regret in non-stationary case?}

\begin{theorem}
\label{thm:prob-miss-pose}
The probability $p^\pi_T(P^i)$ of encountering stable pose $P^i$ within $T$-steps under some stationary policy $\pi$ is given as follows:
\begin{align*} 
\begin{split}
p^\pi_T(P^i) = \lambda_i \left[ 1 + \sum_{k=2}^{T} \sum_{j=2}^{k} {k-2 \choose j-2} \left[ (1 - \lambda_i)\eta^\pi_i \right]^{j-1} \left[1 - \eta^\pi_i\right]^{k-j}\right]
\end{split}
\end{align*}
where $\eta^\pi_i = \frac{\sum_{j \neq i} \sum_{k=1}^K p^j_{u^k} \pi(u^k | \lambda_j)  }{1 - \lambda_j}$ is the probability of grasp success for policy $\pi$ in all poses other than pose $P^i$. Here $p^j_{u^k}$ is the ground truth grasp success probability of action $u^k$ in stable pose $P^j$.
\end{theorem}

\begin{corollary}
\label{cor:prob-miss-pose}
The probability of policy $\pi$ missing a stable pose with probability $\lambda_i = \epsilon$ under $p_\lambda$ after $T$ rounds of learning is given as follows:
\begin{align*} 
\begin{split}
1 - \epsilon \left[ 1 + \sum_{k=2}^{T} \sum_{j=2}^{k} {k-2 \choose j-2} \left[ (1 - \epsilon)\eta^\pi_i \right]^{j-1} \left[1 - \eta^\pi_i\right]^{k-j}\right]
\end{split}
\end{align*}
\end{corollary}

\todo{Ashwin: add discussion of special cases for above for specific choices of $\eta^\pi_i$. Also finish writing out a more interpretable bound which uses the fact that $(1 - \epsilon)^j \geq 1 - \epsilon j$ for $\epsilon \in [0, 1], j \in \mathds{R}^+$}

\todo{Ashwin: I can write up expected number of occurrences of each pose by a particular round for a fixed policy if that would be useful/interesting? We may be running low on space though...}

\subsection{Regret Analysis}
\label{subsec:regret-analysis}
In standard bandits literature~\cite{TS-regret}, the finite-time expected total regret in $T$ rounds is defined as $\mathds{E}\left[\mathcal{R}(T)\right] =
\mathds{E}\left[ \sum_{t=1}^T (\mu^* - \mu_{k(t)}  \right]$ where $\mu_{k(t)}$ denotes the expected reward for selecting arm $k$ at time $t$ and $\mu^*$ denotes the (unknown) expected reward for pulling the optimal arm. 

In the setting presented in this paper, since we have a disjoint set of arms for each individual context (or equivalently each stable pose), the policy learning objective is equivalent to solving independent bandit problems for each of the $L$ stable poses. First we define the expected total regret for grasp exploration on a specific stable pose $P^l$ and then generalize this notion to a new definition of expected regret across all stable poses.
\begin{definition} 
\label{def:regret}
Define the expected total regret for grasp exploration on pose $P^l$ in time $T^l$ as follows
\begin{align}
     \mathds{E}\left[\mathcal{R}_{P^l}(T_l)\right] = \mathds{E}\left[\sum_{t=1}^{T_l} r(P^l, u^*_{P^l}) - \mathds{E}_{u^k_t \sim \pi_\theta(u^k_t | P^l)} \left[  r(P^l, u^k_t) \right] \right]
\end{align}
where $\mathds{E}\left[\mathcal{R}_{P^l}(T_l)\right]$ denotes the expected static regret for grasp exploration after $T^l$ rounds of exploration in stable pose $P^l$ and $u^*_{P^l}$ denotes the (unknown) grasp success probability of the grasp with the highest grasp success probability on stable pose $P^l$.
\end{definition}

\todo{Ashwin: Define regret for $p^\lambda_t$ where dist of seen stable poses is non-stationary and analyze this (probably Future work)}

In practice, we perform grasp exploration on the distribution over the $L$ stable poses encountered during policy learning as defined in~\eqref{eq:stable-pose-dist}. Thus, we need to define a notion of regret which captures the expected regret over $p^\lambda_t$. One way to analyze this problem is by viewing it as $L$ independent bandits problems, where the current context selects which set of arms are currently "active".  

However, when stable poses are sampled from $p^\lambda_t$, the subsequent context depends on the success of the previous grasp attempt, violating standard assumptions in contextual bandits. If instead we assume that the object is re-dropped after every grasp attempt, and thus that stable poses are sampled from the stationary distribution $p_\lambda$, we can define a notion of expected regret in this setting as follows. \todo{Ashwin: Let's try to relax this, or at the very least get some bound on how different $p^\lambda_t$ and $p^\lambda$ are likely to be. The nice thing in this problem though is that these distributions just govern how long we are in each stable pose, within each stable pose it just reduces to standard Thompson sampling...}

\begin{definition} 
\label{def:pose-regret}
Define the expected total regret for grasp exploration over all stable poses as follows.
\begin{align}
\mathds{E}\left[\mathcal{R}\right] = \sum_{l=1}^{L} \lambda_l \mathds{E}\left[\mathcal{R}_{P^l}(T_l)\right] 
\end{align}
This definition captures the intuition that the regret incurred on likely stable poses should be weighted more heavily than that incurred on less likely stable poses. Further, we note that since under $p_\lambda, \mathds{E}\left[T_l\right] = \lambda_l T$ for $T$ total rounds of learning, the above can be rewritten as follows.
\begin{align}
\mathds{E}\left[\mathcal{R}(T)\right] = \sum_{l=1}^{L} \lambda_l \mathds{E}\left[\mathcal{R}_{P^l}(\lambda_l T)\right] 
\end{align}
\end{definition}

\begin{theorem}
\label{thm:regret-bound}
Given the definition of regret in \Cref{def:pose-regret}, we can bound the finite-time expected total regret as follows:
\begin{align}
\mathds{E}\left[\mathcal{R}(T)\right] = \mathcal{O}\left(\sum_{l=1}^{L} \lambda_l^{3/2} \sqrt{K \ln(T\lambda_l) } \right) 
\end{align}
\end{theorem}

Note that this sublinear in the number of rounds $T$ as desired. \todo{Ashwin: add more}



==> notes.tex <==
Animesh
09/14



- Contributions:
   -- Formalize/framing set of problems as instance of one general case new problem family that combines active perception & grasping (done before in some ways, but not frames/formalized in this way)
   -- Claim solving of a particular instantiation of the problem w hierarchical RL that generalizes concepts from prior work and should extend to harder instanced
   -- A lot of baselines to study problem

- Story:
    -- Model free (vs previous approaches e.g. based on geometric planning)
    -- Partial observability (POMDP) because object is not always directly visible
    -- Choice of general purpose algorithm to work for both the current and future instantiations of the problem
    
- Figures
    -- Figure 1: (page 1) pull figure  illustration of problem
    -- Figure 2 : (page 2 top) image of robot doing specific instance, high level diagram of approach
    -- Figure 3: proposed algorithm, training pipeline
    -- Figure 4: setup of experiments, sim + real (early enough to show training)
    -- Figure 5: histogram-like line graph of results
    -- Algorithm 1: main hierarchical learning function
    -- Table 1: number of actions, failures, [put our method on left]
    -- Figure 6: something about qualitative results/thinking for testing, maybe hand designed bins w known optimal , maybe size of heap, 
    

-Formalize general mechanical search problem (is the problem per definition model free?), then the specific instance for this paper.
-Andrey to write out algorithm details in english, should be a hefty section
-Put baselines into experiments section, state hypothesis, then explain hypothesis ; maybe separate experimental setup and experimental evaluation

==> outline.tex <==
-Intro
    - Motivation
    - Visual search -> passive, active, interactive
    - Grasping
    - Combination of visual search and grasping
    
- Related work
    - Visual search in clutter
    - Grasping in clutter
    - Pushing for grasping
    - Mechanical search (combining visual search and grasping)
        - Hierarchical learning
    
- Problem formulation
    - General MS formulation
    - MS for bin picking
        - POMDP of the high level search problem (actions are discrete!)

- Method
    - High Level Search Policy
        - Solution to the POMDP introduced before
        - Paragraph "Learning Algorithm"
        - Training (explain simulation details)
    - Low Level Policies
        - Grasp policy
        - Push policy
        - Paragraph "Learning Algorithm"
        - Training (explain simulation details)
    - Visual segmentation and recognition
        - Segmentation in depth
        - RGB Siamese network matching
        - Training (explain simulation and real world details)

- Experimental setup
    - Baselines
    - Simulation and real world setups
    - Termination
    
- Experiments (only the discusion of the results!)

- Conclusion

